Whodunnit? Crime Drama as a Case for Natural Language Understanding

In this paper we argue that crime drama exemplified in television programs such as CSI:Crime Scene Investigation is an ideal testbed for approximating real-world natural language understanding and the complex inferences associated with it. We propose to treat crime drama as a new inference task, capitalizing on the fact that each episode poses the same basic question (i.e., who committed the crime) and naturally provides the answer when the perpetrator is revealed. We develop a new dataset based on CSI episodes, formalize perpetrator identification as a sequence labeling problem, and develop an LSTM-based model which learns from multi-modal data. Experimental results show that an incremental inference strategy is key to making accurate guesses as well as learning from representations fusing textual, visual, and acoustic input.

==> model_diagram.tex <==
% colours from http://colorbrewer2.org/?type=qualitative&scheme=Set1&n=5
\definecolor{myred}{RGB}{228,26,28}
\definecolor{myorange}{RGB}{255,127,0}
\definecolor{mypurple}{RGB}{152,78,163}
\definecolor{mygreen}{RGB}{77,175,74}
\definecolor{myblue}{RGB}{55,126,184}
\definecolor{mymagenta}{RGB}{231,41,138}
\tikzstyle{every pin edge}=[<-,shorten <=1pt]
\tikzstyle{neuron}=[circle,fill=black!25,minimum size=8pt,inner sep=0pt]
\tikzstyle{visual neuron}=[neuron, draw=myred, fill=myred]
\tikzstyle{source neuron}=[neuron, draw=mypurple, fill=mypurple]
\tikzstyle{sentence neuron}=[neuron, draw=myblue, fill=myblue]
\tikzstyle{hidden neuron}=[neuron, draw=mygreen, fill=mygreen]
\tikzstyle{output neuron}=[neuron, draw=gray, fill=gray]
\tikzstyle{word neuron}=[neuron, draw=myred, fill=myred]
\tikzstyle{dense neuron}=[neuron, draw=mypurple, fill=mypurple]
\tikzstyle{empty word neuron}=[neuron, draw=myred, fill=white]
\tikzstyle{annot} = [text width=6em, text centered]
\tikzstyle{connection}=[opacity=1]
\tikzstyle{conn}=[opacity=1, draw=gray, line width=0.1ex, shorten >= 0.15 cm, shorten <= 0.15cm]
\tikzstyle{sconn}=[opacity=1, draw=gray, line width=0.1ex, shorten >= 0.15 cm, shorten <= 0.05cm]
\tikzstyle{fithidneuron}=[draw=mygreen, rounded corners=8pt]
\tikzstyle{sourcefit}=[draw=myblue, rounded corners=8pt]
\tikzstyle{visualfit}=[draw=myred, rounded corners=8pt]


\begin{tikzpicture}[font=\Large\bfseries]

\def\initX{1}
\def\initY{1}
\def\layerD{3}
\def\times{5}
\def\imgt{10}
\def\dtimes{3}
\def\dinitX{5}
\def\dinitY{4}
\def\src{{"A","girl","eats","a","pancake"}}%
\def\tgt{{"","Ein","Mädchen"}}%

    % T=0
    % Draw the source bidir lstm
    \foreach \time / \x in {1,...,\times}
      {
      \foreach \name / \y in {1,...,\layerD} {
         \node[source neuron] (H\time-\name) at (\initX+2.25+\x, 0.5*\y*\initY) {};
        }
        \node[fithidneuron] (HiddenFit\time) [fit= (H\time-1) (H\time-3)] {};
    \node[below=2em of HiddenFit\time] (x\time) {\normalsize \strut \pgfmathparse{\src[\time-1]}\pgfmathresult};
    \draw[conn, ->] (x\time) to (HiddenFit\time);   
    }

    \node [below=4em of HiddenFit3] (enclabel) {\Large Shared Encoder};
    \node[sourcefit, line width=0.4ex] (SourceFit) [fit=(HiddenFit1) (HiddenFit5)] {};

    \draw [conn, ->] (HiddenFit1.40) to (HiddenFit2.140);
    \draw [conn, ->] (HiddenFit4.40) to (HiddenFit5.140);
    \draw [conn, ->] (HiddenFit2.40) to (HiddenFit3.140);
    \draw [conn, ->] (HiddenFit3.40) to (HiddenFit4.140);
    \draw [conn, <-] (HiddenFit1.320) to (HiddenFit2.220);
    \draw [conn, <-] (HiddenFit4.320) to (HiddenFit5.220);
    \draw [conn, <-] (HiddenFit2.320) to (HiddenFit3.220);
    \draw [conn, <-] (HiddenFit3.320) to (HiddenFit4.220);


    \node [source neuron, above=3em of HiddenFit3] (s-attn) {};% at (\initX+2.25+2.5, \initY+2) {};
    \node [annot, above=0.5ex of s-attn, text width=12em] {\large Attention};
    \draw [sconn, ->] ([yshift=1ex]HiddenFit1.90) to (s-attn);
    \draw [sconn, ->] ([yshift=1ex]HiddenFit2.90) to (s-attn);
    \draw [sconn, ->] ([yshift=1ex]HiddenFit3.90) to (s-attn);
    \draw [sconn, ->] ([yshift=1ex]HiddenFit4.90) to (s-attn);
    \draw [sconn, ->] ([yshift=1ex]HiddenFit5.90) to (s-attn);

    % Draw the Imaginet decoder
    \foreach \name / \y in {1,...,\layerD} {
       \node[sentence neuron] (M-\name) at (\initX+2.25+7, 0.5*\y*\initY) {};
    }
    \node[sourcefit] (SFit) [fit= (M-1) (M-3)] {};
    \node [annot, above=0.8ex of SFit, text width=4em] {\large \strut Average Pool};
    \node [below right=4.5ex and -4ex of SFit, text width=14ex] (enclabel) {\Large \begin{center}\centering  {\sc imaginet} Decoder\end{center}};

    \foreach \name / \y in {1,...,\layerD} {
       \node[visual neuron] (V-\name) at (\initX+2.25+9, 0.5*\y*\initY) {};
    }
    \node[visualfit] (VFit) [fit= (V-1) (V-3)] {};
    % Arrow from the Average Pool to the Image Vector
    \draw [conn, ->] (SFit) to (VFit);
    % Arrow from the encoder to the Average Pool
    \draw [conn, ->, draw=myblue] (SourceFit) to (SFit);
    \node [annot, above=0.5ex of VFit, text width=6em] {\large \strut Image};


    % Visual attention
    %\foreach \ix in {1,...,\imgt}
    %  {
    %    \draw (\initX+12-0.1*\ix, \initY-1+ 0.1*\ix) node[minimum
    %    size=2cm, draw=myblue, fill=myblue]{};
    %  }
    %\node [rectangle, minimum size=2cm, draw=myblue, fill=white] (c54) at
    %(\initX+12-0.1*\imgt, \initY-1+0.1*\imgt) {\LARGE conv$_{54}$};

    %\node [visual neuron] (v-attn) at (\initX+12, \initY+2) {};
    %\node [annot, above=1em of v-attn, text width=12em] {\Large Image Attention};
    %\foreach \ang in {1,...,5}{
    %\draw [conn] (c54.30+\ang*10*2) to (v-attn);
    %}

      % Decoder
      \foreach \time / \x in {1,...,\dtimes}
      {
        \foreach \name / \y in {1,...,\layerD}
        {  
           \node[hidden neuron] (DH\time-\name) at (\dinitX+\x*2, \dinitY+0.5*\y) {};
        }
        \node[fithidneuron] (DFit\time) [fit= (DH\time-1) (DH\time-3)] {};
        \ifthenelse{\x > 1}{\node[above=2em of DFit\time, text height=2ex] (y\x) {\small \strut \pgfmathparse{\tgt[\time-1]}\pgfmathresult};}{}
        \ifthenelse{\x > 1}{\draw[conn, ->] (DFit\time) to (y\time);}{}
      }

      \draw [conn, ->] (DFit1) to (DFit2);
      \draw [conn, ->] (DFit2) to (DFit3);
      \draw [conn, ->] (s-attn) to (DFit3.270);
      \draw [conn, ->] (y2) to (DFit3);

   \node [above=0.5ex of y2] (declabel) {\Large Translation Decoder};
\end{tikzpicture}


==> nn.tex <==
\begin{tikzpicture}
[   cnode/.style={fill=#1,minimum height=3mm,minimum width=3mm+2pt,box,inner sep=0pt, opacity=0.2, text opacity=1,text width=3mm,},]

    \foreach \x [count=\xi] in {1, 1.4, 1.8, 2.2, 2.6}    %%% INPUT
    {   \ifthenelse{\xi=3}
           {\node[cnode=gray] (v\xi) at (\x,-2.4) {\tiny{$\mathbf{e}^t$}};
            \node[cnode=brown] (b\xi) at (\x+2.4,-2.4) {\tiny{$\mathbf{e}^{b^t}$}}}
           {\node[cnode=gray] (v\xi) at (\x,-2.4) {};
            \node[cnode=brown] (b\xi) at (\x+2.4,-2.4) {}}
	;
    }
    \node[rectangle, inner sep=0pt] (v_word) at (1.45, -2.7) {\tiny{span embedding}};
    \node[rectangle, inner sep=0pt] (b_word) at (1.45+2.4, -2.7) {\tiny{book embedding}};

    \foreach \x [count=\xi] in {2.3, 2.7, 3.1}                   %% hidden
    {   \ifthenelse{\xi=2}
	    {\node[cnode=green] (h\xi) at (\x,-1.0) {\tiny{$\mathbf{h}_t$}}}
	    {\node[cnode=green] (h\xi) at (\x,-1.0) {}}
	 ;
    }
    \node[rectangle, inner sep=0pt] (h_word) at (2.7, -1.3) {\tiny{hidden input representation}};
    
    \foreach \x [count=\xi] in {-0.3, 0.1, 0.5}                  %% softmax & softmax-1
    {	\ifthenelse{\xi=2}
            {\node[cnode=blue] (dpr\xi)  at (\x,  1) {\tiny{$\mathbf{d}_{v2}^{t-1}$}} ;
	     \node[cnode=blue] (d\xi)    at (\x+1.7,  1) {\tiny{$\mathbf{d}_{v2}^t$}} ;
	     \node[cnode=blue] (d1\xi)   at (\x+3.5, 1) {\tiny{$\mathbf{d}_{v1}^t$}} ;
	     \node[cnode=blue] (d1pr\xi) at (\x+3.5+1.7, 1) {\tiny{$\mathbf{d}_{v1}^{t-1}$}}
            }
            {\node[cnode=blue] (dpr\xi)  at (\x,  1) {} ;
	     \node[cnode=blue] (d\xi)    at (\x+1.7,  1) {} ;
	     \node[cnode=blue] (d1\xi)   at (\x+3.5, 1) {} ;
	     \node[cnode=blue] (d1pr\xi) at (\x+3.5+1.7, 1) {}
            }
            ;
    }
    \node[rectangle, inner sep=0pt] (d-1_word) at (0.2, 0.7) {\tiny{descr weights $t{-}1$}};
    \node[rectangle, inner sep=0pt] (d_word) at (0.3+1.58, 0.7) {\tiny{descr weights $t$}};
    \node[rectangle, inner sep=0pt] (d1_word) at (0.3+3.2, 0.7) {\tiny{descr weights $t$}};
    \node[rectangle, inner sep=0pt] (d1-1_word) at (0.3+3.2+1.7, 0.7) {\tiny{descr weights $t{-}1$}};
    
    \foreach \x [count=\xi] in {-0.3,0.1,0.5}                %%% Descriptor matrices
    {   \foreach \y [count=\yi] in {1.8, 2.15,2.5,2.85}
        {   \ifthenelse{\xi=2 \and \yi=3}
              {\node[cnode=red] (R\xi\yi) at (\x, \y) {\tiny{$\mathbf{R}_{v2}$}};
	       \node[cnode=red] (R1\xi\yi) at (\x+3.5+1.7, \y) {\tiny{$\mathbf{R}_{v1}$}};
	      }
	      {\node[cnode=red] (R\xi\yi) at (\x, \y) {};
	       \node[cnode=red] (R1\xi\yi) at (\x+3.5+1.7, \y) {};
	      }
        };
    }
    \node[rectangle] (R_sym) at (0.1, 2) {};
    \node[rectangle] (R1_sym) at (4.6, 2) {};
    \node[rectangle, inner sep=0pt] (R_word) at (0.05, 1.5) {\tiny{descr matrix}};
    \node[rectangle, inner sep=0pt] (R1_word) at (0.05+3.5+1.7, 1.5) {\tiny{descr matrix}};
    
    
    
    \foreach \x [count=\xi] in {0.6, 1, 1.4, 1.8, 2.2}          %%% OUTPUTS
    {   \ifthenelse{\xi=3}
            {\node[cnode=gray] (r\xi) at (\x,3.6) {\tiny{$\mathbf{r}_{v2}^{t}$}};
	     \node[cnode=gray] (r1\xi) at (\x+2.6,3.6) {\tiny{$\mathbf{r}_{v1}^{t}$}};
	    }
	    {\node[cnode=gray] (r\xi) at (\x,3.6) {};
	     \node[cnode=gray] (r1\xi) at (\x+2.6,3.6) {};
	    };
    }
    \node[rectangle, inner sep=0pt] (r_word) at (1.45, 3.3) {\tiny{reconst span embedding}};
    \node[rectangle, inner sep=0pt] (r1_word) at (1.45+2.6, 3.3) {\tiny{reconst span embedding}};

    
    \node[rectangle, inner sep=2pt, align=left] (loss) at (2.5, 5.5) {\scriptsize{\begin{tabular}{l}
                                                                                   {\bf if} view($\mathbf{e}^t$) == $v_1$\\
                                                                                   \hspace{2ex} maximize ( similarity ( $\mathbf{r}_{v1}^t , \mathbf{e}^t$ ) )\\
                                                                                   \hspace{2ex} minimize ( similarity ( $\mathbf{r}_{v2}^t , \mathbf{e}^t$ ) )\\
                                                                                   {\bf else if} view($\mathbf{e}^t$) == $v_2$\\
                                                                                   \hspace{2ex} maximize ( similarity ( $\mathbf{r}_{v2}^t , \mathbf{e}^t$ ) )\\
                                                                                   \hspace{2ex} minimize ( similarity ( $\mathbf{r}_{v1}^t , \mathbf{e}^t$ ) )\\
                                                                                   
                                                                                  \end{tabular}}};
    
    
    \draw[->] (v3) -- (h_word);
    \draw[->] (b3) -- (h_word);
    \draw[->] (h2) -- (d_word);
    \draw[->] (h2) -- (d1_word);
    \draw[->] (dpr3) -- (d1);
    \draw[->] (d1pr1) -- (d13);
    \draw[->] (R24) -- (r_word);
    \draw[->] (R124) -- (r1_word);
    \draw[->] (d2) -- (r_word);
    \draw[->] (d12) -- (r1_word);
    \draw[->] (r3) -- (loss);
    \draw[->] (r13) -- (loss);
    
    
    \node[rectangle, fill=white, inner sep=0.5pt] (label1) at (4, 2.5) {\tiny{$\mathbf{R}_{v1}^\mathbf{T}\mathbf{d}_{v1}^t$}};
    \node[rectangle, fill=white, inner sep=0.5pt] (label1) at (1.6, 2.5) {\tiny{$\mathbf{R}_{v2}^\mathbf{T}\mathbf{d}_{v2}^t$}};
    \node[rectangle, fill=white, inner sep=0.5pt,align=left] (label1) at (4.7, -0.3) {\tiny{$\alpha\times softmax({\mathbf W_{v1}^d}[\mathbf{h}_t;\mathbf{d}_{v1}^{t-1}])$}\\[-0.4em]\tiny{$\ \ \ \ $+$(1-\alpha)\times \mathbf{d}_{v1}^{t-1}$}};
    \node[rectangle, fill=white, inner sep=0.5pt,align=left] (label11) at (1, -0.3) {\tiny{$\alpha\times softmax({\mathbf W_{v2}^d}[\mathbf{h}_t;\mathbf{d}_{v2}^{t-1}])$}\\[-0.4em]\tiny{$\ \ \ \ $+$(1-\alpha)\times \mathbf{d}_{v2}^{t-1}$}};
    \node[rectangle, fill=white, inner sep=0.5pt]                (relu)   at (2.9, -1.9) {\tiny{$ReLu(\mathbf{W_h}[\mathbf{e}^t,\mathbf{e}^{b^t}])$}};


    \plate {pair_view} {
      (d1)(d2)(d3)
      (dpr1)(dpr2)(dpr3)
      (d_word)(d-1_word)
      (R11)(R12)(R13)(R14)
      (R21)(R22)(R23)(R24)
      (R31)(R32)(R33)(R34)
      (r1)(r2)(r3)(r4)(r5)
      (R_sym)
    } {\scriptsize{\bf pair view} $v2$};
    

    
    \tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,below left=3pt and 0pt of #1.south east] % 

    
    \plate {input} {
      (v1)(v2)(v3)(v4)(v5)
      (b1)(b2)(b3)(b4)(b5)
      (h1)(h2)(h3)
      (v_word)(b_word)(relu)
    } {\scriptsize{\bf input}};
    
    
    \plate {single_view} {
      (d1pr1)(d1pr2)(d1pr3)
      (d11)(d12)(d13)
      (d1_word)(d1-1_word)
      (R111)(R112)(R113)(R114)
      (R121)(R122)(R123)(R124)
      (R131)(R132)(R133)(R134)
      (r11)(r12)(r13)(r14)(r15)
      (R1_sym)
    } {\scriptsize{\bf single view} $v1$};
    
    
        
    \plate{loss_p} {
      (loss)
    } {\scriptsize{\bf loss}};
\end{tikzpicture}



==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

